Can Features for Phishing URL Detection Be Trusted Across Diverse Datasets? A Case Study with Explainable AI

Phishing has been a prevalent cyber threat that manipulates users into revealing sensitive private information through deceptive tactics, designed to masquerade as trustworthy entities. Over the years, proactively detection of phishing URLs (or websites) has been established as an widely-accepted defense approach. In literature, we often find supervised Machine Learning (ML) models with highly competitive performance for detecting phishing websites based on the extracted features from both phishing and benign (i.e., legitimate) websites. However, it is still unclear if these features or indicators are dependent on a particular dataset or they are generalized for overall phishing detection. In this paper, we delve deeper into this issue by analyzing two publicly available phishing URL datasets, where each dataset has its own set of unique and overlapping features related to URL string and website contents. We want to investigate if overlapping features are similar in nature across datasets and how does the model perform when trained on one dataset and tested on the other. We conduct practical experiments and leverage explainable AI (XAI) methods such as SHAP plots to provide insights into different features' contributions in case of phishing detection to answer our primary question, "Can features for phishing URL detection be trusted across diverse dataset?". Our case study experiment results show that features for phishing URL detection can often be dataset-dependent and thus may not be trusted across different datasets even though they share same set of feature behaviors.

==> methodology.tex <==
%\vspace{-0.2em}
%\subsection{Problem Formulation}
%\vspace{-0.1em}
%For phishing detection, it is expected that all the features across different datasets need to contribute consistently within a regular value range for building a generalized model. More precisely, it is not convenient if specific features in a particular dataset with a certain value is helping to detect phishing instances in contrast, the same set of features in a different dataset behaves quite the opposite. To address this issue, we resort to the state-of-the-art XAI system SHAP, which provides us with the top contributing features and their corresponding expected value ranges for a specific prediction or classification model. 

%To illustrate, if we consider two phishing URL dataset denoted as $D_1$ and $D_2$, then we start with pre-processing the datasets and find the unique feature set ($F_{u}$) and common feature set ($F_{c}$). Then, we create the merged dataset ($D_{merge}$) based on the common features across multiple datasets, say $D_1$ and $D_2$ in this context. After that, for both dataset $D_1$ and $D_2$, we generate statistical measurement based on each of the features in set $F_{c}$ and do a pairwise between datasets comparative analysis to assess if there is any innate deviations within the common features' value ranges. After assessing the feature statistics, we proceed to train the ML models with all the features in $F_{c}$. Next, we conduct some experiments in different settings (details in section \ref{sec:evalaution_experiment_setting}) to compare our model performance deviations. We further use the same experiment settings for SHAP \textit{Explainer} along with the feature data from the two datasets. SHAP (i.e., Shapely value) provide the features' contribution for different train test settings through bar plots and summary plots presenting features' contribution and value ranges, respectively. By using the intuitions from each of these dataset specific plots and comparing their corresponding feature contribution pattern and value ranges, we can find out whether the feature contribution deviations present in those datasets to ultimately answer the question {\em ``Can features for phishing URL detection be trusted across diverse datasets with similar features?''}. 
%\footnote{here we can try to establish the justification how and why XAI make sense to apply in this problem}
%\footnote{this section supposed to be more mathematical or specific rather than subjective...after reading this, one should get an idea of input and output of the system...}


%\footnote{current fig 1 is not clear...it's not a system architecture. you can think of it as a illustration to show our research steps....it's confusing in its current formation}




%The main motivation behind our study is our hypothesis that the features' importance or contribution to model prediction across different datasets varies even when applied to a specific problem (ie. phishing) with the same feature list. We also hypothesize that some specific features, only found in a particular dataset contribute more to prediction than the common features usually seen across different datasets.  

%\footnote{Figure 1 needs to update illustrating the current methodology}


%\subsection{Data collection and pre-processing}


%\subsection{Dataset balancing}


%\subsection{Feature analysis and selection}


%\subsection{XAI models}


%\subsection{SHAP explanation on cross-model assessment}

